Event-based Navigation for Autonomous Drone Racing with Sparse Gated Recurrent Network

Event-based vision has already revolutionized the perception task for robots by promising faster response, lower energy consumption, and lower bandwidth without introducing motion blur. In this work, a novel deep learning method based on gated recurrent units utilizing sparse convolutions for detecting gates in a race track is proposed using event-based vision for the autonomous drone racing problem. We demonstrate the efficiency and efficacy of the perception pipeline on a real robot platform that can safely navigate a typical autonomous drone racing track in real-time. Throughout the experiments, we show that the event-based vision with the proposed gated recurrent unit and pretrained models on simulated event data significantly improve the gate detection precision. Furthermore, an event-based drone racing dataset consisting of both simulated and real data sequences is publicly released.

==> temp.tex <==
% Comparison table with three significant.
% Let's use two significant for the sake of space
\begin{table*}[th!]
\tiny
\caption{Comparison with existing methods on the AU-DRONE dataset. c: center error, d: distance error, o: orientation error \IB{Fill the table} \IB{Why is the caption format different?} \IB{We should remove some columns or find better representation} \IB{Do not normalize}
\label{tbl:comparison}}
\begin{center}
\begin{tabular}{|c|ccc|ccc|ccc|ccc|ccc|ccc|}\hline

method  & \multicolumn{3}{c}{single gate}  & \multicolumn{3}{c}{multiple gate}  &\multicolumn{3}{c}{occlusion}  &\multicolumn{3}{c}{partial}  &\multicolumn{3}{c}{distant layout}  &\multicolumn{3}{c}{too close}  \\ \hline

  & c & d & o & c & d & o & c & d & o& c & d & o& c & d & o& c & d & o\\
\hline
\hline
ADRNet \cite{jung2018perception} & 0.046 & n/a & n/a & 0.096 & n/a & n/a & 0.071 & n/a & n/a & 0.052 & n/a & n/a & 0.085 & n/a & n/a & 0.044 & n/a & n/a
 \\
ADRNet-mod \cite{jung2018perception}  & 0.071 & 0.147 & 0.046 & 0.151 & 0.356 & 0.106 & 0.125 & 0.345 & 0.078 & 0.098 & 0.227 & 0.065 & 0.133 & 0.386 & 0.109 & 0.087 & 0.189 & 0.080 \\
DroNet-mod \cite{loquercio2018dronet}  & 0.165 & 0.188 & 0.103 & 0.500 & 0.602 & 0.428 & 0.373 & 0.452 & 0.287 & 0.131 & 0.179 & 0.091 & 0.509 & 0.599 & 0.337 & 0.087 & 0.144 & 0.146  \\
Morales et. al \cite{morales2020image}  & 0.213 & 0.314 & n/a & 0.580 & 1.227 & n/a & 0.391 & 0.870 & n/a & 0.229 & 0.782 & n/a & 0.512 & 0.930 & n/a & 0.156 & 0.172 & n/a  \\
Darknet-mod \cite{redmon2016you}  & 0.103 & 0.122 & 0.058 & 0.207 & 0.244 & 0.126 & 0.147 & 0.248 & 0.09 & 0.154 & 0.142 & 0.081 & 0.192 & 0.216 & 0.101 & 0.109 & 0.159 & 0.070  \\
\hline \hline
\textbf{GateNet}  &  0.050 & 0.100 & 0.050 & 0.160 & 0.249 & 0.129 & 0.150 & 0.390 & 0.129 & 0.074 & 0.143 & 0.060 & 0.116 & 0.183 & 0.108 & 0.058 & 0.110 & 0.077 \\
\hline
\end{tabular}
\end{center}
\end{table*}



% Second version
\begin{table*}[th!]
\caption{Comparison with existing methods on the AU-DRONE dataset. c: center error, d: distance error, o: orientation error \IB{Remove some columns}
\label{tbl:comparison}}
\begin{center}
\begin{tabular}{|c|c|c|ccc|ccc|ccc|ccc|ccc|ccc|}\hline

  &  &  & \multicolumn{3}{c}{single gate}  & \multicolumn{3}{c}{multiple gate}  &\multicolumn{3}{c}{occlusion}  &\multicolumn{3}{c}{partial}  &\multicolumn{3}{c}{distant layout}  &\multicolumn{3}{c}{too close}  \\ \hline

method  & \#  & speed& $E_{xy}$ & $E_{d}$ & $E_{o}$ & $E_{xy}$ & $E_{d}$ & $E_{o}$ & $E_{xy}$ & $E_{d}$ & $E_{o}$& $E_{xy}$ & $E_{d}$ & $E_{o}$& $E_{xy}$ & $E_{d}$ & $E_{o}$& $E_{xy}$ & $E_{d}$ & $E_{o}$\\
\hline
\hline
ADRNet \cite{jung2018perception} & & & 0.04 & n/a & n/a & 0.09 & n/a & n/a & 0.07 & n/a & n/a & 0.05 & n/a & n/a & 0.08 & n/a & n/a & 0.04 & n/a & n/a
 \\
ADRNet-mod \cite{jung2018perception} & &  & 0.07 & 0.14 & 0.04 & 0.15 & 0.35 & 0.10 & 0.12 & 0.34 & 0.078 & 0.09 & 0.22 & 0.06 & 0.13 & 0.38 & 0.10 & 0.08 & 0.18 & 0.08 \\
DroNet-mod \cite{loquercio2018dronet} & &  & 0.16 & 0.18 & 0.10 & 0.50 & 0.60 & 0.42 & 0.37 & 0.45 & 0.287 & 0.13 & 0.17 & 0.09 & 0.50 & 0.59 & 0.33 & 0.08 & 0.14 & 0.14  \\
Morales et al. \cite{morales2020image} & &  & 0.21 & 0.31 & n/a & 0.58 & 1.22 & n/a & 0.39 & 0.87 & n/a & 0.22 & 0.78 & n/a & 0.51 & 0.93 & n/a & 0.15 & 0.17 & n/a  \\
Darknet-mod \cite{redmon2016you} & &  & 0.10 & 0.12 & 0.05 & 0.20 & 0.24 & 0.12 & 0.14 & 0.24 & 0.09 & 0.15 & 0.14 & 0.08 & 0.19 & 0.21 & 0.10 & 0.10 & 0.15 & 0.07  \\
\hline \hline
\textbf{GateNet} & &  &  0.05 & 0.10 & 0.05 & 0.16 & 0.24 & 0.12 & 0.15 & 0.39 & 0.12 & 0.07 & 0.14 & 0.06 & 0.11 & 0.18 & 0.10 & 0.05 & 0.11 & 0.07 \\
\hline
\end{tabular}
\end{center}
\end{table*}



%%%%%%%%%%%%%%%%%%
\begin{table*}[th!]
\tiny
\caption{Comparison with existing methods on the AU-DRONE dataset. c: center error, d: distance error, o: orientation error \IB{Remove some columns, but which ones?}
\label{tbl:comparison}}
\begin{center}
\begin{tabular}{|c|c|c|ccc|ccc|ccc|ccc|ccc|ccc|}\hline

  &  &  & \multicolumn{3}{c}{single gate}  & \multicolumn{3}{c}{multiple gate}  &\multicolumn{3}{c}{occlusion}  &\multicolumn{3}{c}{partial}  &\multicolumn{3}{c}{distant layout}  &\multicolumn{3}{c}{too close}  \\ \hline

method  & \#  & speed& $E_{xy}$ & $E_{d}$ & $E_{o}$ & $E_{xy}$ & $E_{d}$ & $E_{o}$ & $E_{xy}$ & $E_{d}$ & $E_{o}$& $E_{xy}$ & $E_{d}$ & $E_{o}$& $E_{xy}$ & $E_{d}$ & $E_{o}$& $E_{xy}$ & $E_{d}$ & $E_{o}$\\
\hline
\hline
ADRNet \cite{jung2018perception} & & & 0.04 & n/a & n/a & 0.09 & n/a & n/a & 0.07 & n/a & n/a & 0.05 & n/a & n/a & 0.08 & n/a & n/a & 0.04 & n/a & n/a
 \\
ADRNet-mod \cite{jung2018perception} & &  & 0.07 & 0.14 & 0.04 & 0.15 & 0.35 & 0.10 & 0.12 & 0.34 & 0.078 & 0.09 & 0.22 & 0.06 & 0.13 & 0.38 & 0.10 & 0.08 & 0.18 & 0.08 \\
DroNet-mod \cite{loquercio2018dronet} & &  & 0.16 & 0.18 & 0.10 & 0.50 & 0.60 & 0.42 & 0.37 & 0.45 & 0.287 & 0.13 & 0.17 & 0.09 & 0.50 & 0.59 & 0.33 & 0.08 & 0.14 & 0.14  \\
Morales et al. \cite{morales2020image} & &  & 0.21 & 0.31 & n/a & 0.58 & 1.22 & n/a & 0.39 & 0.87 & n/a & 0.22 & 0.78 & n/a & 0.51 & 0.93 & n/a & 0.15 & 0.17 & n/a  \\
Darknet-mod \cite{redmon2016you} & &  & 0.10 & 0.12 & 0.05 & 0.20 & 0.24 & 0.12 & 0.14 & 0.24 & 0.09 & 0.15 & 0.14 & 0.08 & 0.19 & 0.21 & 0.10 & 0.10 & 0.15 & 0.07  \\
\hline \hline
\textbf{GateNet} & &  &  0.05 & 0.10 & 0.05 & 0.16 & 0.24 & 0.12 & 0.15 & 0.39 & 0.12 & 0.07 & 0.14 & 0.06 & 0.11 & 0.18 & 0.10 & 0.05 & 0.11 & 0.07 \\
\hline
\end{tabular}
\end{center}
\end{table*}


%Backup of current abstract (v1)
Autonomous drone racing is a comprehensive test-bed to evaluate the reliability of a drone for agile flights. To have a successful mission, the drone should have a real-time and accurate gate detection system that allows the drone to locate gates in 3D world. Therefore, unlike standard object detectors in computer vision domain, a gate detector should detect gates in image plane in addition to predicting their distances and orientations relative to the drone. Moreover, a gate appearance changes significantly during the flight (e.g., gates are observed partially before the drone pass through it). In this work, firstly, we propose a convolutional neural network-based gate detector (GateNet) that detects a gate center in an image plane, and its relative distance and orientation. Unlike similar studies, our method achieves state-of-the-art real-time performance on an onboard computer. Secondly, we propose a gate detection dataset (AU-DR) that closes the gap between computer vision and drone racing. In our dataset, we highlight different cases that appear during a flight in drone racing. In our experiments, we compare GateNet with similar studies and show its superiority. Moreover, we demonstrate the effectiveness of our perception network through careful experiments in a realistic drone racing setting. The code and data will be available at \url{{https://github.com/open-airlab/GateNet.git}}



% Backup abstract (v2)
Fast and robust gate perception is of great importance in autonomous drone racing. We propose a convolutional neural network-based gate detector (GateNet)\footnote[1]{The code and data will be available at \url{{https://github.com/open-airlab/GateNet.git}}.} that concurrently detects a gate center, its relative distance, and orientation to help locate gates in 3D world frame using only images from a single RGB camera. Unlike similar studies, our method achieves high inference rate (up to $60 \si{Hz}$) on an on-board processor. GateNet is also very robust to gate pose changes and background disturbances. The proposed perception pipeline leverages a fisheye lens with wide field-of-view and can detect multiple gates in close range, allowing a longer motion planning horizon and smoother gate transition even in tight environments. For training and bench-marking, we propose a comprehensive dataset (AU-DR) which focuses on gate perception. Throughout the experiments, GateNet shows its superiority when compared to similar studies while being the most efficient neural network for gate perception implemented for autonomous drone racing. We demonstrate the effectiveness of our perception network on a fully-autonomous robot in a challenging but realistic drone racing setting.


%Backup
Drone racing is a suitable benchmark problem for agile flights, featuring a light-weight quadrotor with limited computing and sensing capabilities flying at high-speed in challenging scenarios. The developed technologies can be transferred to expand the reliability, operating range, and flight time of drones in many applications~\cite{pham2017distributed, bozcan2020air, bozcanilkeruavadnet}. There is still a gap for an autonomous aerial robot to match a human pilot~\cite{moon2019challenges} with difficult challenges in state estimation, motion planning, and control. However, a fast and reliable gate perception plays a major role in the system's overall performance. 


\begin{table}[!h]
\caption{Success rates for gate passing based on eight trials for each case when changing a gate's location and orientation.
\label{tbl:experiments}}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|}\hline
 \diagbox{Post.}{Orient.} & \textbf{0}$^{\circ}$ & \textbf{15}$^{\circ}$ & \textbf{30}$^{\circ}$ & \textbf{45}$^{\circ}$ & \textbf{60}$^{\circ}$ \\\hline
\textbf{0.5 m} & \cellcolor{Green1}100\% & \cellcolor{Green1}100\% & \cellcolor{Green1}100\% & \cellcolor{Green3}75\% & \cellcolor{Green4}50\% \\
\textbf{1.0 m} & \cellcolor{Green1}100\% & \cellcolor{Green1}100\% & \cellcolor{Green2}87.5\% & \cellcolor{Green4}50\% & \cellcolor{Green5}12.5\% \\
\textbf{1.5 m} & \cellcolor{Green1}100\% & \cellcolor{Green1}100\% & \cellcolor{Green3}75\% & \cellcolor{Green4}50\% & 0\% \\
\textbf{2.0 m} & \cellcolor{Green1}100\% & \cellcolor{Green2}87.5\% & \cellcolor{Green3}75\% & \cellcolor{Green4}62.5\% & \cellcolor{Green5}12.5\% \\
\hline
\end{tabular}
\end{center}
\end{table}
% GateNet 31,580
% ADRNet 2,511,932
